SPANet: Generalized Permutationless Set Assignment for Particle Physics using Symmetry Preserving Attention

The creation of unstable heavy particles at the Large Hadron Collider is the most direct way to address some of the deepest open questions in physics. Collisions typically produce variable-size sets of observed particles which have inherent ambiguities complicating the assignment of observed particles to the decay products of the heavy particles. Current strategies for tackling these challenges in the physics community ignore the physical symmetries of the decay products and consider all possible assignment permutations and do not scale to complex configurations. Attention based deep learning methods for sequence modelling have achieved state-of-the-art performance in natural language processing, but they lack built-in mechanisms to deal with the unique symmetries found in physical set-assignment problems. We introduce a novel method for constructing symmetry-preserving attention networks which reflect the problem's natural invariances to efficiently find assignments without evaluating all permutations. This general approach is applicable to arbitrarily complex configurations and significantly outperforms current methods, improving reconstruction efficiency between 19\% - 35\% on typical benchmark problems while decreasing inference time by two to five orders of magnitude on the most complex events, making many important and previously intractable cases tractable. A full code repository containing a general library, the specific configuration used, and a complete dataset release, are avaiable at https://github.com/Alexanders101/SPANet

==> 2106.03898v3_Shmakov/.git/objects/bf/2a990e3a6622386958680aa70e3c53d0c0c676 <==
xì¼w<×ýŠŒB²G¤²"R$Ù+QÈ."Œ¯™Ù"YÉÌ(#ÉJȌ¤P*##…Ñ s}<¿s^¯óï9¯óßy^ÏÓSùŒ÷¸ß÷}Ý×}Ý닗­wJI––$‹Ô×Sg å¤%##cÐÔP1$#£0!þ£¡Æß<µ¿5"ÿQº+kž¢Á?~4¶øó
Sw22«â?ò/ùäBøK'ª	éäe{'—•›™———¸ƒ³"»•‹øe·ó·çå9ÉÈv'iª(òNÿ:ìE2›ÌP\_É(z}á"çÁ³7o›Ù֜æ¨bïæe}¶åZ7¿íñ€k7ÜQêyV|4é¬A±…'ÂTc˜qgK£K"ê|½–óÃ}ƒ³kÈùµ¦ôéàã‹ÅC©=õ=þ
/·Ä__VK{ýdÊ=ó<§ïÌûó™ËuÒso…\¢©éÉ÷³c%;}ùßVü"0M©O5Jb)x´r$çõdœâº÷ñËëvsgG[§î܎¹°¤x×A†Â…~¿S¼ihNcøë'¾£¿×ž|à{bÝä;ÊæV©ñi*Bm¡æCæ.<öá-ñ¸ÎœŸZáû•X8;³mÉ$=`yÈ}{Nã²ï6œqO^^HûÙªÎ{å◼WS<¨fêiyé¦of_.WιÈz¿¹û™·†3EªøþPÌNó\ø·òÎF[|}ô<í[º…#F}*«•k´z:#ž)ÚÆAqÎMJþŽ"ç~b''/;ww? g|j´c¬¹ ´¸®—ïÒ¦ýSG>þ‰ßf&dR*¿b¦GóŽÖòUÞ?c77)-ûž¶ˆø]Ë/õTTTliûºÊ]×|¥e./
Þ{¤Áw%MììŠúñ´Ÿb¾B§kB¨Ç^^Y°«!Þ¦-Ê}˜Ù+p¹˜==e ïòTÓتÃÊ¿×A[¿Í,uz.fr§§">]Úýîâ!F,(Ó«7oBwG³Mì&íòÈOòþYñôÿžýú_ãîI'Ç9d†}E»vàÒתq9[<¢QÈ\xø1*àCáÝ5›ðŸŽf#§»«F¢ÆBC]£´ˆ1‹‡wu~[YùØ°Ôlu{0ÃÁÝáÃê\³¼ó¶efÄKÍUÇ
¾Ý»wú£œ‰…\ºòOFaµ§Ó|guFY¹¤/Mç5Ä+ÚjÈK7¥ž‰ËæäqìË~ݵR¯¥y\˜²û—ògJŽ½må«xQCC#â¤ñƒß½åÎUß°Ù4Z»ºk(ù*ž]°â;­çüX˜øyF¹%ñؙªhüD㼘	†®"gÓDü°—ƒŽ?ŒiR†FÚ'UñÃܬþÿoýÿ|™ûþ¶"æ¼îµá%ì\þ_,ÿuµÈÜòÿ|Ce8woØÄÞÿ›‰˜Æ¥ÐDF,'¨­MMúàÁ¬¬,r]]Ý—.©^¹ò'ôܾ}û.\¾¬~ö,׳±ýÁM;kkkÉüjͲ*+—6L,6:Wm"cÞ¾œlkø¦-[¶'U
^ÏÍ\õSܽ›g'íÙ¿…õúù†Ë°ÐþËxAAa¡'‡ÇÁ¢âbƒ³g£ÃÂÂèìŠÊË%÷8É]1_[öON{ñBÇÖÞ^`×®‰gŠ›)ÈñÀ™ï>¾0èé"å,Ɨé‡C:;µÒå<hïÈT32ÚáèèÈHO7Á áä$zæìYSÓ÷Wäy))ȉGíÝ»ùׯ_==íw•BFIréÉ/®áôˆ7—Û´»Œ·lÙxž^†2Æ'A'fš››"õù.¨wGþWjÜàÜÏ–'à`ŠO""üŒ44»wäX5	<,HNfå>êË¢ËÝô:GÝuiÚ ]1ÐB.YXE€é"±qöÇÌyyyl
ó˾úúA¸ÆæSG<ûa7Á'¥–†7Ÿ«Ú2UVVÊzÛ¹•[6èxøÖ±¯ï+zãû>|ˆÚ´yëhãÕMddº}û/¼ÚÃ{"3Gíú³Žø]ñûÒoFŒ_åºÎ,\ôøñÏgÑkW7mÖ?{V"ç¹[öëéṔv¾@z2
]ÝV\opêÔµ-Û÷ìÜ»W]v7S+L"Š&TY–4Íøs~8zn°jbi¦¯7¾`óTOf{ò¾³ev]¬dÇv26®.NH:ÉêÜÚOΧ.ËÏ4s•*º£ÅÑÉ©ü|ï×á:¶:¯µ+WêH'³9>œ¹oVÃ,zºäÚ°s{Ó®ýv,1\2[1¯¤Xu•µÌWj¯^zãçîÛå>?ìõ
Y¶Gªè‡=|(E–©W•¯{;ìæMævIŠ´ü-{³G¬›¤®bË/~x´‹)ëþ9†Ä•@¼Ê¤œBÔøþ155ê|½Œ(â6îÃ7í¢;Fa-ô³ý…'Mê<÷ºô¡…jöZm­œß·¦Í«£!Ûi(õ

ƒM+ì­:nð÷¾Ž(Ø¥î}÷.'ëå܇ʂ''±Ç©`§»µ"-ŸßÜÝñòeÛ}ӊo5=þ±\Ì4t¬ñeúB×°r6¸á]ý•*;/Ý{ë…EEÏÆ[£_Y°ªv5)³$ÇØhÃCG"94skk9±>-³oŠ_
‰ñ"ëˆs^·î¹sô]ÅùmO,$ì_¦GÞ¾ü"ÃÇÇ#‹Ä·Hs¶>õÿSæ6©uq¸v‡¹¹yo¼†ÒƒØ°Ë'"JÖ}_Ü9Êå\uVŽ3žp;,›§^f4w&‰–;¾I?â¥'·Õ´cq¢}q¶¸tüºÌHãòÀ¹¸Ûε[zË#ÛqËq##£ÕoÍۈ[HžžZíütNMWêÃ'»Rrrs)«†=¹$ø˜[éX
è"'¬°0ïjÜ÷JÔ$d]k¶º¶j뗷šr\þÌUÙôæjŽÞQr'*ïžø€e…M´Çi·ó×æcÇÿ.ÝSTUR"w®_6NLLü6\ ã[ªŠô±x
J®C±'ææûxÂzôÒe¯¦Xøn	üÕuî[¨"9«XPßLb¬ª­#voåºZ9löɯϷe¯ü¼OâÎ&?â5ÏðïÏG›™Þ¼êå·gË]ƔY÷eÀ¢fs4ƒ{{
Å,ž°cÚ½®¤ÓçÎÆ-ƙ"[S=]m•°^ÿû«lp«£J]'ýZèóP"ÌG¿íÄÖ%%%[KŸþI–8{d¾zS…}÷¸µw¶Å¸ZŽJ}Y࿀'ë¿¿˜=ÑK&ýüjúdu<Ú{eØËuÀÜË
¶)vFe qëk£tÎË
k‡]ã	Õ0³³Û}çÊüaz>Š´tty»˜8X±äÛ899¿½={Ùj¸Ö#}šÙ||úuÎêb\`̯SóujZZQ$Af¸¦Z
Aæ&u>ÿk
ëË¥ðæ)±ÇmM^_`)>]ªæà ̺ï̵ÁË
^ÜÌæp…Ó|?çÃÿŽm"õÿýˆÄ"Ð7==Ýøqý§LžÚ룿Ìç©»x";MÊ:¾Ã/¶+®3ayc•mÏ,//¯.—^¯t¿º™·q´)#ŽÄ*wц*s.¿ø^êš2ÿŒ¬ŠÖ»†@Å;~ß5‡þÌ­>c{ÚØfk*fb«iggç½üæ´ÏáBԈ;¬18Œ£Yá¼Êñ$Áìj@m‡Ë—ÛÏ^®mø·¶ðäÈ
¡6b0K}'lš'©VgO7ÐƵcœBÎÕ¯…LÛ^fY¬û¸¶ì5ˆۅs6ٙôî©ÿ'§X›zã#ƃ·‹ZhkÓmXÊDÛuâÒ/ý€	\…Oñ›s:71bš+Ï*føx¤â¿Š.^ÄÜUÈ‹¨¿²2Ža>ƒ¿É›`l¥§c.¬¨Ø~ùÉ"õÀ&}<›ØPâ€nSXÝÉÌ̜»‹i&–*:Ñãï¶÷çór_Ý?×À‹…X}éõ4"i—šF;o'®Y¼…@<͈ï—}WÛík¤"áýþ6ü[ùWfûœYﶦpºe<óì—/‹ãÑÙOž˜ÉÑ2-ÀàH"	ß~ä㯭Wƒ°Šä"Ñ:—Ûcy¼¿?ßkZ¡3èà=[x¯ÞxFHe cþŽH•2ïEkù?_+.88ÄÇW':hýÑ£7`q…!^CEn«AƒkŽTÞïß¾±îãýQÅÆ"a½¼þK¹ùùð³ôÊ:`üƒUXõ-,bùÖ¦ÕeÝ>EX²°Ÿ'M+w¬ÿÈÌ©¬4 [›jܧ¾ñý[ä3y|1•¸hÌüš-m–>MiýOη¥ç$xB#ÆŘ#G	ö<aïâõË~›·Çüú`¹eü؛7o
ÝiŽÜ¾77‡1þ.Ž8q¾âŽþd¯rÛÙ<±[YêÑ÷ïnÖ¸"n…"Yˆfœ`X¥ó°œüÚRŸ|Aj"BN^Õ¿åsÿBuoÒTç¯`"J¿ ՊÌC¦áÃJ6o¨2?±"×Ç.G8•uèÀ-®Ì"Cԓ£mvoê¶Áoðk¾C毩è@"g`+…Šç¤9×^"ôüRÈü¥ê8pàmÿµ?
|‡¸ÎSÛr]H¤Ï©¯çiø;)Q×2#$MÀ/ü«wo»Þ½À[âƆðQ°¼ýÙØ·ÐÀ­¡Êlë)/f&âÕÌÍyx}>1	

¨(àx8Tüýü¬ÈÌzøÐPŽvù&FØ5Ü7smp.¿i«ÞIŠS·O<±þŽJŽÁ5å,º99¹WïßGºÈrOåöóÕyÎ=ë;¡x@ƒ›ˆ#®&e#©Î{q çîÓ§r´æW1åÁ¹õoÄÛ/¤Q§tQ¥t-§ÆyyxdáŒðððÐP‡ÀٌNª…46üûÓ0±Yq•ÜÍÍ-wâF+ö´ *ŠVþNjœ"c•Ù\å2¾yË#_
œc­´·Û¾'ŸŸŸ8TCS"üÛ̙¦ù‡;è©_¿/œ~³öÍÀÀÄ̶̽í'ä¯6…lFÜ¡«˜?¡Ëì5ýŠü	×hí³5|B9KKC£Œ"5ËÞ|hȓ|•toñçOÏGUU»Øé¿?Ì.`þ;¸¾w}òÜ:UsCBìqÖÖÌlAë•ùaïõ_S¿^žÓWV¦çÝ|,Q'¦æoS5¨x²Zîȑ×##±oß"H$š{ùøÝߕÀ2OáÇlúz];'MʄæV®¥œHýb2®Ó'í-Ïë]o_ßÍyÎhtÎZt%ݼéfUûØãÉãQN]9µ°RÇ.ãœNâ~È^i\xsìÒȓÔI'—
ÅU²ï?~Ä'%…bZÉŲ³wœác²îÞ%KMMÕÐÑIŒµãÀFxÿ|¾üÒà¡![É¡ÍÑãöð…Þ"I§'(ìæQõq®âRÈÜfQzº¦ní16¬Þ8÷ÑãÇÙyy¡)L6bÜ['ZÙε4oSŒÀDîVŽ¢K.~ç.ËýÍ·þÛ/?¹Œ^×iߞGn&$ħ§ÇCEKËȸ×ríBؗhø+EVfk`Vfiðâ0_ïîË&%ւ''Lϟ?ÇÞ÷d¦ëíííí½'œìiUôæíÛ=<ڇŠˆáŽºÕì÷ùn;#›+kqäî­µ¢>";žŠ¤vÛOñýû÷II­nyŒ¥Ñ÷~÷îÐoÖH•op ë5Ðpõûløâë»òMõKÌ]I±x¥""ԍÌ̸¥%Òüé¼ýáÍä
ãž<'_]°øùÆ@–»NâI`͌Pî~V±¨H͟nø½£+IoÈYæáÇû½¿Y"Mj¾³¢þ›Èú55›-±5TUƒûx4·`VõÆÚ´ÇÂߨÂúçEDD¾}­è`¡ÕT—¬oiQùôù³€ŒLJÕϾÐö㞞‡$è¾ì"uÞð‰â`ë}ƒP²X'¹Fßd©/Uè#ϋëݬ•Ž'V†µ_|«Dĺï	™£Dža !)f'{;,ŒzŠ<™@bé›7~ÿþ½˜1Iw8%ÖÝÝ=þƍ<í8¹¸q°G‡jÜq?<éuooðù;>Ô½:Ïç<›V~¨ÞüÝ:ç¹yŒó…£™kúWSw®l=¡ðKðãÐ
qÙ¦lrºPåÕI‰ÀÈç_j¨KòàØÛÙ¸…ræÙĢ嫻J/^|2_Ó70 p_䕟ñâ&eŽÁÅÁÔ?fQ.ª|VŸžWž]SS³×UCÒ¢"-dó65__¹Ù¹ó:ϱm«!$zC2:V†Žº…§Ñ@íû"pˆÛ"……ýsn͎ļúN:èô)'X¥=ˆk]'Ԟ¬Œ\é•Ôižt㗑a»zŒÌ³Îx)Ž:R7w÷šÇÛF¼'.~|j.GÊNǺÜ5Ö¾øÁ©t1,¢;}â'~®R¨[ÃpKü;/'¼|ù9¯O¦œkCf˜—sCsÑTÍßøäɐsÇن4±Á‹HÂd÷îÕVç§ø6c׬Bíúï¾Åôׯ-‹týoßj©óo·nÊV˜d#"4NӌP˜}Õ`|jj$ìÛb«`³«,wGg§²½ý¾ÌW,lÞWϞÓÏ,·4È|ò󃓬Çl"‰þø—§!]_–ñÄÚ¢ùv'ÛúÚí{õF«Öè¥8œ¥µê®ÿY°ùñ¹»W'¾ž—'æ[/]jgkÜ ò«yr*.g++~V1"<¡:ÀV³ID;Wõ19ÖÊd˜Kþ¡Y¼©O½=§tD¸Æ¹Ö/¥
/UúÄLHº°¢
 ©!(ÀÓê"­òqAÎË»ù™Jþ˜‹ìŒŒn­Òð3¿¦2§RCûEqŸàÄÓU´Û·órØõVžcSâHIp/ééÜÕfâX>dw"g½,;"fR6]DÀ©S§NÁҁ#vIHÄIË"ñ÷¯RXd:Nò¤
½'DB9å9?‰ÁD.,K–{ë`±÷ÒkuŸ+G"{ì+ÆÆÂùÚžþ<¨0"±ˆß[>¾"MÊ
ԁ?7 ­úŒjo_ßb3ß:£ÌKàMu-2"Å–í'¾¹­îÞ0ë¬,%9j:Vó=@90
5'§bK3»'Ÿì: ÈŽæðm)±Ê'ÙeeŒD¶ò‹»šà=ç|Ié(¡ëɟù:Y¿Õ2}ó­£W}¬ßN®¡­ÝL"@ +-uÉLŒÈ…1¾ ñºRyÎëßÞå'÷fìJޗkEsè6ƒ×°›óÓ_ödCA)÷gzÛë›Çq,"°žÄšøY™<ñ–ŒŠŠÒ××ÇN_[Z'¥ŒG4÷ž«XÝ´=sDiy:'ÎBè´Ê')'¦üь>±Òîûk2Åǂߟ³üöûKiªYþ~WlQìÆñ!Qøä·þ"'šV´Õ™N…Øc>fRFCVveÅy^…UÃÆå—ûOr/o_6P ²‹OŸ>i¨3UÙws~ª9‰¥¤c͘#҆<›.äÌw|g…Áòæ÷և>¿Á<7'âÏÜåÀèüü=3ì¶db&×þ­}ü׊ä
·ˆˆ‹ '<³g/OhG¢Ÿ_À·>Ë·${
T*=EB«DÝlçzöñÅ&ð¸+Mځ™€ÃâowsÞ½vÒoáÊÇf̯ú€lØsadOȵrKS"³goO~tÐÍTà‰"ÿN"®wYØnÙ=¿?ƒÛ^¤Èˉøݗ¹~Ír¿O%îxG`{à'vkû·®^øq[ÞæºÆyìݶ£KŒ%uór3BÖDNðsð²vûN¥"KÒ´.ÇUE…$$ª–ÌCܧ^¶nÚ&jiÕ{omÔº'¢´n3±ÃÀ·@Í'S›‹ŒŠ÷۴у‹Q–£Ý2JÙd¹ŽäÌc"i¿(×d¿+qµMæéUÄlÓuµÅÁë¬Yú¸Å²éá]ä°|ç_¦ÇÇò[#áZ½ø{o²h¶ìÌ[S]cðwÆ÷Mø1¥2KS#£$»Ît,ÚSýgöÍw"î`X2OtÒe
ä¢"ÀDœý©û i1©
	ú"âY73s3³˜Ëþ_Κ½Òlq®šÈü÷+SÒw錐+ÛÖð}íw`½:ºmgvWÛFçÖc¶d€ÎÈnífóç"u	jŸ6¡§KV'A½'ã⢢t(w¬ŒzÖÙ3'¥t…"¥fAlì5Ÿï–ù¨"˝«äú,؎‰Ï‰	Ld®MKRÏT³MÜѶ‰Ëô{"…·ÀeÈææ´éê2(üžÞ5ÃβW̄õÕ»wjBç€\½ÿ.¶ìFrã{#>þ*撏d;'·HVüóF¤úuÕ_˜æq'f‹©&–ü³LC$<•Br$µPrO¸Iù¥WǽgòRÄ~˜1àNex}CVnŽüƒ}¯IÔ×qÊCßíäÙU2ÿä‡è<ø¦ågŸž'¸"C×n(^þ20?öJ
µ™"±¬4¬¿'Z '¿âGf˜"@¢˜
áºü"Éýó‹øX&°	ÈÜö-W¼Âõž£äÜòÞúrjC,¬¬€ª²æòÑÅjúU–ó32Í¡ÇJ®b&QQj9på˜Ë⟵՟U
ÝõHE;gHãÈTcóæÅü0¦Ã­†ìtÉلÛÝ Œ"舍ÖÐÓC& ²éFZZÔåÀ?ƒ.²¾OþiÜööÁÙ<ý˜2Ka»tO~Äâ5_Jêöû­ºÌ°«äiõ(ÇMÌ`¡~…—`{é£ÈYŨ''"Ï|¶|íЗo5ö,´W2BCŽM¼+'gÓ¢
CÝ hB¬ƒ¨´%Ç\ص"Å°
l0†!í0
"³<Äþ·öæicèŒ2œF: Zpqzß‹é«»ÛE
è56˜ó¬Zýý´WÑ`ýïÓ´4΋ïʚÏ™ï5¡™}†äO'g—øÓ¥<	~	‰Ø®ÖW¯²Ž»¶óxi´GDÛu%Ÿ|F¥Í¶Ê¹²åêK ÆV™¡<!㖘ƒ¸xr,";I•s‰¾—‰.Yø	|•8Ï®Ï7oÞü¨£Ü'
'Ȳ9-±]ÝÚ:›"xëÊ¿µ•Vm~ì¾{»ç¹ýF¯nƂ‹ïXX™xúg>g``x÷øÒm<|¾q–ù?kiiíwèÄzZ¶ÅpÜ:t)³ñLŸ‰XAŽm߈Bxý!÷ž£Äz¿ò_¾÷7'!))	Äô
<"œ.™BK[{€îʟ¯_±@Z¦Ù¾S@	p/Ù;g'VK}'O™eêÐLß½ø›7ƒâ¬ß•Yi‰¯ß'u÷JŒ˜~c²®ÙƇªË|zr»yB¨#¸®§
Õz|AU€œ̺²žÞV'G³ýÔ¨e#¢ï‰¼Æ¾XãsÇú#ÄõXFRýYsǞö-ɑ•[<–4Gnaߝš-€t-Ëö÷¯q¶†'¿it³\È$üg´{%­b7È#¥M֙~ß·ÈóöØñ
H3PQQ!^?.ìù."$ÔøÄçG®
c<¹ÿ¼{f3lZt"XžÁ'çÚ¼"ÄO>=pÐëÒ	Œò'C±ÞÕf%²»ûÂóªžþ±¬Xä×RIé"fXr»ùE¯îy]rûÔ-ösõ:Ž@'HÆꑄ¼Kæ2/'"Í@ՀO.ÀQ—*ÃA±í‡1ç#rV!QVog¾•gö¤©›,7ì«
UTnln]V]œ7…¦6òx
e-:(Ÿùê‰I™NhŽŠúí{î\ǃÙ~ÌV®žÚÁ´c¡u®›;4Ã.yÑì¬ã{ÿ¶6¿Ð¼âÕ®»€þ¼¾]{ÿjÞMï¸Ýöì™2"P—ËÔo;[[K0µ°Ÿ Î c;áãöÀÊ7Ø¢ßW©ºlñzÒàDçÔ+L£æÕ·êëÃ]­ÎId€Î¨^û9ˆcJØ
0»ËYÚQêˆç×WIù]]Çž;;;]~/9¯Ï?唲¥Ùsâ΋v¾ø«·&7%ù
¢f"KbAlJ@þ눭l"T*pË'½c— àm@þZÓ©Á7éõ
Mj¨´e;¤õÊ´»"×ý®vnØK0ÒD¤;™ j¿K½mîS¼/°Ö~ûìX&"Œõh·ßU°l'Š9ÕjWk[5(éØ/èÚ2w‹3ià£Áß_u+iNU‡Býì&V±í‡¯ü¼h¦xKnöò ·Œ3wkECfÄ}›–¦N½òÇßð\ýDÕ%fõJ½{ݝqג¬¢ÙH°¢í‹Ø"ʴ䨗™é'5/Ž<9œ2×I6öS2௷y•»bÀ"Þ͏™
þ2€ÃÎQƒÚƒKˆ=VûaF…)%ö%­™ŠçªÜ.iòÜdbò«ÈÝÕBI—ìƒÅhÄr1xܵ˜âÜÊ#DzK-æ•$Óë{j±Ü…Ÿ>¼	º{å·!"çÁ«<G<Ù¿ÃAƒ³ß
~"¨ìºxs/ð_òYç1›ë£/þr›W»ð)}Ôh5ŒXŸ'²—'¤¤É»ô)•S4§±Ž<J¬w´Åññ5ÛªØz$ìэzß}øæã˝gǝvˆ™P{·DVÏ©dô?:ð-ŒËy´dN…å$°BFblV²¡tYWe9jóMtÉMsÃu§—曞N+¸ÌÕ :ž©­¥õ,†ãÀø­˜ˆû³µ_Jôs×Ã
Ë-9ÌÌÍ3H×Üë†o¤¸v÷÷=iµðFD"´LºY½½oÚ+IªrŸ¡!1`Pˆ"‡7üãtÕ±A‡Ý?û}6;ŽÒáåù1Ìc7Ò¶"Κʗ.íÛ@*¯ŒÊ,9༭ªÝï{d:¡´¦v'…M´f:1"F"'F¨fq•§Ü]›<éáÉëï?e†ôàÖa÷|€Ô‡w7'ŠWÃëkòþ»ìÔ~véµ¥YC02·ŸK‹P|\rå8 $*z\ˆåf¬ÒéÆëjŽÿÖ×6¨,Ѻá­uÃ/ÛÙâ#¾ûU¾¿($,Ü´Ueß°b?âyŸÄ2‹èHíñõäMíÄ6r›¹ãÌT{¤ÅYÅB	®ún±¾P‹ûæH
Ô_YÃè9xŽŸ3ik
¶;†'ØIg›'ˆ834**—ͯÈàop86}@iÂL<…D?ºS'CΞŒ)ÿDfɃJº5Çvºdr#cc-õWFêê›Á>Á=35}YÎ.(А+éìêÊÛ¥¿Í¤Œ¾ 'ç¸\p	Á·S
dÓÁKˆñ(aÉ£À KJÂz¦b³DßÜbŠ¯¹Î§hQØu
‡BÝß¿žD_ÛoJLIiv®Òn¥{þü=·ÛpÝî={¬	¢P'äñ©ƒ	;¾jÿùž;¡ƒsɱY·AJ)܉ÐÑy3µ«™x†;ŝLæ׶‹… r''ÅÁ>h¨ï¨}ѹݪ¢ð³7.#žæÁkN{ÁÉ餣'­
%6§¥À÷êª÷ èþø1<4‰	ëtØou¿<o։06âaI±€t²«1ºä«Æ\'ƒ*Ìs5b:**::o×tÔàAv:üTúÐ!,£®,÷ç÷!*¶Pê܀tY\%ÍR¬ Î8tûrw12™Çç;hÍÍÌöÛ-ü–Þ…ÕӟšŠ‰¡'öo@šð†4µNNÍ0ADEE>±bRGèÔsb8FÅí *X—7¾$Ü|àó³XÉ%؎q#¹{Ûrċ:@)*‰ÉÉùý>…€É±Çþ!23Šìs9mǬ®òVßÄDˆGIF¤ÞTæF€ªy/)§·NIÀ0S‹*z»Øœpå~š"®Ý<Çe6Xác*ýN";îÃ[' a§d;^PT¤L`+zsÔV­Áo!bEøv/¬ìÚ½[U.L¼}QQl
4†"¯"[®ÓKOÅV
â¼°¹ëZÛݶâÚç`´µÕ_1ôð	
0œ=³=؎¥`\"pû¶(V» çTšå›þ~ì³KŽÁqPE§¬ÙVÖ'ú±x<—±X>3œžƒB·/quáAiééñ†æ¯²M̬×ՒW"æä"@ ґˆx>¶ò'Ïf:»¤DOŽâ*•6ˆ¿©xœÍ¯]EÅ>9!aÁòÆeå#fòº€$a(ä(˜

ËÈ*ïH‰²ŠY‰Ýö#ûºÌEÇ:I¥}Kë<£[ˆ€Ô¤ù`û&Ìd÷ýtå'Å°}W¸>L"`%#¬ÛfHZêÅ_¿^´;äkïµízނrDî®é윜f7؄"h,î¾`âRI1Ì»¸"Ü7£âèX"/³|^ñ¶¢=èÔá3mE^Œ.BâOТiª¹dFoo>´|>¡–"‹ôÂj¦]×ÚZ€––"ei­œ@ñÑÒRR.«ß¬fØ7y®ÿõéò_ˆ	Û.¦"''Ñ©sôԻȀ»²ÝR
VYKgNŸ†Ѷibî¢ß0
6³ð¥ÀÚ{¦ÓSãDêj`œvÎÙĪ(]ºt©"Ë5l6´OLÀÝÐ.˜ê¿Ý»N¥­oc"#å5S°t\óDº=Sj´V«˜©ã"ÚÛ§ÜÝ+H"æ0/½²'`ÜúG(,ßþ¤¬OS¯Ie¡›¿<m¹ìÅ=S•¶)ÙÄÃ|ÉTÚ¬tÉ;ôŽLeˆÔ·;°Æ/~ß'BcWn¹ÅЎÍköˆ^EDŒvÒTžÈiÍQ\×iQÅíŒÉþuk¦nÞ!yà‹ª‡G¥TÝï"3÷W‡ŒíÎ5|þl¯ð/\ŸR'ÙwY߯3ýÚ.Gtûü1QrÖ­Ä+i"ßlõ‰¥*Árm5¢5&€¥ƒ˜Ið)Žá‡–3ᘪg±ýÏÆÊH"Ä
æj5ÚÉøæŒJGk$‹lÃä‰ë…MÌBvpáÏõí'[¹ÎÛn½ÊÒB &cÞÁ(óuÍÖj§ÄdYØ錿'sü45åžiD'ΤiÙÆ="wϗ4EmCàq`5à.ø^'Šu@]S©È/ãÒ¡ÛRÿöÙ¿:ÚíxáÂ1ì‰Û0}Gæ`Ë}}!Û癋BRÂF¼«éù-|xayNçne=âÁ¯ƒ

Yº#œ*"–îuRF;•Ù.
	ˆ™<"©HñbߋX¶=¾½ŸX륬ÎOêIšé¦‹ÅIÁyá´¸ŽS&âôüEU4uðu,PöúÉ<K×àÝÑçü•ŠäW9BÄ\<ËgD˚¹ò°ß;t¯A¾P˜SaHþ9§î`Ãe8óÈ'ì=ÛŽvkéè¨èê^—'ØÉrÅØϹXªi|Ï«‡?AÙ%GÕ2
È'ÞA¥}CdAì"OÕùf·UIDE!X|ȹê{Ó)àe42gʀ÷urrJˆ½
Šk†&9¿Mô‰fáC¥óêêá$ÊÙ½˜£øÀ‡"ð"cÎÃv¹¡ÄDjÒ¾ö&øúʇ"©l¬Þ·3ü,«óŒTñ"tôôI·y	k6,ƒ_ÈÝu#£,&"¾A,"'éýÿ°>¥ÄÝö…×SBàŠ¤÷¬ãs¹%ÑB;{Çþ ´ôÝòr¹­[Ê>|QÂ!5¤êrü¨¸klZ	j ›ÌÛÖ1zÈá4ÛﲏIGßÏÅő™]d7ÒÓÅþ;NÁ"åá‰ùàb•$Û*Mm©*0s.'Ü8s¿ü6Ä3¯Bµ§;1Ô7ÿsÙ{Mbyùù"åÔtd[½KŸÛ5MµÈ0Ïòýœ'ªi3ìÉmÁ»;À«3G¡†ŠD+®à	;0v
õWª¦Ô½Pâ0í7z,«ðäÕ+TIÚÂ:pîùɉ7Ã-DºÔ¹ŸÇh¾6k³8•Õékøt,®U'ixhعŠÙK¥·Ñ%MÕÕ®Ä÷×{"|†.œ2!B¥yõ°ó)##«o£M¨ð˜¬H‹¢è†\¦óþG"¢õ¼éG¯§¶;ùúÖæ=õRkْ\,ˆÑÓÍØcÔÏXS¯k)6ÿ
h Qváø²ÒP&Ö<Êï×ïÝ6`ŸJÜ/ì¼Lxé'Ëà4Q\ÎQÕ֎&QJ	éUtÐC⇰"#fòݤì–"2Di†½VßnŽ¢•úž©-	;e÷v%¬à!G:|Á'ÓKÉâþˆ>$քÜèµA`†6qìLTgDQÇeQZ;©~´cèԙÀ¤øx~ž«ˆö4Dõˆˆêۄ£Ž¢,ˆ¢ž^!ÅÉ#QÛÚÙå+kM˜©}eQL·gâV0Ã\VT ¤ ã·=>§¨H+R;¸×ï¯~6åö»YYWU‡ÝÿîgüÀÒtò½mº%Ç1OÏÇRg¹qEÿ›7à3Æ¥£ñÛ¬ÂBM`–	ôHOA—̏RƒÝcYDAYß%$æR‡Kº³½
|A'´^Ò§¦êÚyªZþ݃ü|59
á >±(¶$Z˜Çæ@G•3g8‰3ƒ N€R
ákNBoQRDØ£ê'ErJ0úv´pë"tü3‹£m\—[.U
ç÷?Þ#Xúàr(•ÿ°Å:²é¨^%™NϻȺ|ÅÎäF (°l•ÀŽ¬øéï7¥ÙÕÕ&r¬Â"¥ðÈ<È$Šß˜³" ɆŠ…Ü^RVïå›c¨×z~}×%îãó#Èp,å¾ËŽv#·nÄ 'ª	¤xæLšT)¿(ècB§†š(od‡¡Ÿ¹|e-³^Ņ»Hø'c¢aØ÷1µêñ•?I¿>üñSH?ìö…¼à"™8Rhq–b§£|øýçžÌ8þãa–ÝiÓí[ƒD|Ý>¿àÈ{ýyrRxmMŠK¯Œ^PQ'oÌlÉmï¨zb®wŽÖóRbà¢DaPâžiÿÞ¢;&)»LÝpǹB¯" Åz™:(ñž=zéP£l–ªœkƒ®¨üÂkúìÞÛǐœ¡¼÷?\íZ7L€K¬õ­[ª(BXnJ=c¾oà'ó-\+E)y»‰p4µ®5fïê¼Ja;ëóOãšwA	šøþ
#YØ6>qž«âMÁvûQ5vŒ·ÎcvËDçAɵ>±Ú›(b}ߔY5c‡vcüö«ßƴ̍Ýå2äåÂÉüä*QÂ0|÷íÿÖ¿^¤òè¦Æ-ÉLÈScP¡#8iúaˆ&G"
?zœx€:w‹œYÿŸŸÂîí‡Èlmmw@—Úl‰t ˆPžPl‰Oۘ#e—qh¡ž£FþŽ…AMÖºÔ
_pt&'¦lQ…%-ª3´oFzh@;tîWçé2Ôi¿~l8'k¥šcÐì¿@];›œœÄz÷;ùôa>Aj1ìYý& Ý;ëmrEëV·*Ýë晊ò¾—uy:!n
+©n¾…Ր=Lȶ>ŽB™i±ÒØß:ÞR¿IÑÿÒѨŒ#^DJvÈðäIpÏD¨UÙå€B4!"R{!µa£÷³ "R8>6«å^mõ»¢ðO`²ò<=¼°‹å6á}@oco*/
×ÕTjý—»ê‡††ÊzͧÍB-,\éþðMª¿£ÇîtûBaæHˍb#iÒ­¦z½%Gz0éÏìO~L@ô蕟í;y
¤7FÑï†C›çÌK¡PÏß96íz€LŠ¬Ò¢iGBJʽ~Ù³}ÒÐ3Ÿ'£f*:Y,:&­Íƒb"ó^éCó!v–6m1M®&}ȒAlÀX:::nÄ*ûC
J0ŸÇçv8!c©F±¿Ì¡oO×Üí¼g+µååL`
o'1ÈQ^\3؁,>ôýFVY‹€¯õ4á"éJ¿ã³k['o1ÄY*Û-•zK¸jýÀ'#\Ø^js*˜~¡ì̖Pey²'06—aþNÊEY'NTTêâ†ÜÆàÌžã^(¤Ä€‹wœ-XAĽrúؓŀ]ò @ò‡'È@yÑcåÄedN×SùÕVØʾýž1 rr9Lê¾y±\Ø<ür¯×·"1å)¿,mÔUGê¯äÙ¼R•­œåÓ«ˆq£QPZš'©n¤Úw-°ÉWÇÇ­!"Ñj.ÀÿÆÂ7®ivòNoïÇÇ2n"a«˜Éž»³vÏS"ŬÒÏÌD÷‰M@‰ÜHˆÙl¦Åwíڄ|¨W²€
"ªrkݖ9Ï#ÛiÇûE<e»oVAµ;C#)é:®2CÓ¯=t¡_°í:Wx÷m™]‡›ÊE• åބžGî"\"Šâ Ÿ>+—ÿ8zˆp‡/3¢ÿçóë_\nkoÇ[ÿsð''à–Oœ¸±],ܕ«é‡Y¾ŽÔŸ•³C€$Ȩô3­+ÒÅeG¡½LÖÙP]=vì?¾0\ô×ËÖ/ËãP•÷J&~†ï·zFçxÇé%©´»¥eÐÉyB²³)6N¯µõ÷OÏ{™
p®tl;…µFܾºÈ–ùÿñœaïï펪Gõ嘜²xwçK)¬ãÍ[·"xøí1çDóü¡'áV¤E=·ò)ÄҚöˆHØjÞ¹M§ÀGJ©ªª"Gkwõ¥µ?+¢>[NQÜ3nÃƯ+üýv«z2v¬ª:ž|¬Ãn‰íAÚKÌërmnqÞ3þüÌ!9äyHÂÞZí[2{‰#'ÖºIŠ|5"Ø%³8cùc]dÅxZe+¥$ô*¨÷°ÐZµFíÍnÿ{i¦ìýªÛ¥CcS_awP —
ª©ªÄöüg…Iœ²Ý³
PÚfB5è_þãx–7åý»o"Ôà3']ǁ‡QëÝKè9«
µÓ¤Âm¨O»¢b7#h?%\çt"Œè/(,,û§ðjÈ ªÈهXÃoÏ÷fB(!(YwÇ<!PÙ Ædþ"¿g:PfÝJKè{Ù%€BÄBÀBÄBm ›\
ß{X"$)Ô–T>Bñrõ³ÛT÷ô2·±cð »µÚïB -%ŒEƒÖEøÈ!O¸FHv	"ÃN}Ïøm‹ƒqþômäʂ🌫¤úDÞ[	A"€úLP™;033ƒ:¤?ÇGû£d»ß'äÄ`©±Òm"n®®uÏË-So
|ÙàϘN}ÿ•úÇú£ÄÛÞރÚ:qäË*ÉÆ`~ÈÙS'Áì TC±";üŸ"FïÁ´Ö}…î3m#{éê6CW‡@†§›Enº‹¢ŠXÍóÃu(10Ü3îç2ΰŸ{W~ü—»6˜êh':`—>&fB{KÞG
ðµžôO`­7rùݟe+³Ÿ>ì•.ëJ'HAÝ
Ñ1)ö˜Ü¨Z-û¡‹ìÐ
æ.-ÿ†™ù¡–L«wòìރs­Ç{ýØN² ¥Y.lHá»8'N%bv¬ŠçF±¨äûåG"F03órAé'åm(,þC®8Ï¿üˆ
 ¼½½5ê'l;'§¦&PE5tK«ôZ°ÐÛ1º¤Åƒb!¢¢( Ì3€°&épxù•oª]'ªßF'&<ë$Ï¿ärëÚ×y¿[.p]:o1Ô"¥ôüj4¹ULõBZ,A€{«¶zd!愞'Þ¥	w½BoO¥ÚC&4ùï1x$Þ:‹V#"å|Ô쥶œaԙÀíïåÉ9‡uó6´J«œÔæ¾
¸k
1O¹¥p‹}ED4D¼×ÒqHC(Ú`-µ2]U
_ÈuËy̲—˜	£Ë*nFsûºÄs'1¯"'8ã[Xº Rûós.ÿݦ˜"¢Rºh•"D`Úéêœ4"²õ†ŒtÉÖµ÷LD܆ö=ÊÃç÷í*)¦Jé˜6ú¾ûàãª>pmhÓÇÇ¡'™ZÒRú+r]%%¨™°%íۗëÊ¡÷ £#6VaÏ¥þ^ŒÏgC…ù≈ˆ2""¬|'Xuõ"'·ÇrÛ§ÝAl¿#hcÈ.ýÄã³àQÇЙ҂6Œï¿:OøšÕãx[	QÃ@ðLþmçà|‡¿¦Y;õÊXÂ1O®´Î~^ô&ªµHŒ#?»Ô˜AcÊ
2÷p¥@ßþ^é/ ½×–ö•ÏӒ5£÷/L¦FEÚ -Ÿ(µÕò¦ZÙ«ÏhÌmJÆÉç8`ïò`GªñŠ´t3™ŠÐqõ®WôNYÌEš§§imšß}kNR¬úbÍ='÷$ièUŒøLñ¤+ø˕dž440`›rmô鱉Î#O|ÆS^Ž«'Ô'êKÊiH‹ŽPjj÷ÝG±eòǃ3•´¨ãEtMIQÀ§ çESŽº'qØä*û*'z	}¯õÂH½ä?3™'š_Oø¨äOÁZwnÞ†EÁ7öהäÍ"÷´±ñ*°>2ߎóD©¦àþýXü†Ù!wàڗsû~P3®.Mõ=¥6ä†È%¨g
º¶Óë4Ñ ¤¾~¨¤#rô L­Bâ"û—|9…Ð…ýø…Y÷´`™]'œÌ°»&4ADIÙÝݍ›¦À®BP90ô.IXeÔ¿ô0¸-2œ•4hš	{Æ aب²l—öbñ¼H
µ¶X) 2"õiv±M5ïˆzlaA(øq~Lº¼ÿ1Ã0ÀU™ß/·.ó¨RiÈH.U34|t"‰@¨}®DGŠšU,ºcÝ÷ë¥$ð	ŠÛ/¶¾VQë{û6ìÒàã¦'€"Ä6(F"ñ'îWë'"Ïb^éÐäè8:Š ¼ˆ––Ö=É&"	Î5ÿ<š,oºôûE¿¤Ý(¿=Cµ‰"e_ë2(ô	îá	¡ê
†'…TœïÑjg$jÿyÚ)m™Z5ϟߋÆïք­'ï÷š7CÔö¹¨ƒv6dƒ¹67ÈXÅèPÀ¾%eµ{¡5r"=tp°¥1·šw_|çÒ½lÖ µµ•/ʌÁ)¡É§ÙíK÷ôI¨wŒLL"\d/>¿iUñž¢¤ï
™B¼ÁM–¥oZAr®Žhd;tû×¹;¨¹B;ŒªÊµ[ÿ˜tÖ<ûteLfå;€·ýüÌ+›ºœö¹Omÿ9&t)£NGßÛªŽer®£žaŒ êzé[–ÏpÐ6Fõ<YÌ4X_H'\cÌ©O+ùþË54%W×ra‰rׅ£µ_
œòB®na?èȲ•W>Ø!
•eûÍÝÚ._T}ß,ðšŒ¼PösºÔԚXXð"å$®.*^1IÛoEÒ=`H73s¥{ëè'GC'rlXDÈÉMžú&Øcª!ꌞsv$8ôµž•c_ÓՇ@G'<!ôATÑ7ä`œ™7+ÓFd_üwdvvÊ¿T-UU*4C2þÐöà½uàüVêm¼;öñ@
–RC~¦ß  ¾Ðð×.oþZî::IÈ'?½~ûÖþW¼'D¹"Žž
©óK…úSÄ}P(®¿ü°¥HšˆF—}'¾¾âŠ˜X"´{MÁªl~4U}5eÓÖÕUõñ9Œ@–Õñ
Y:V©ãA©@ÅpéÖ>,
!'Dž¾ó{œ–ý½>Ült€FɂEB
=肈#yxX¡M{œ}8æa^H·}s†×Há—ñ)EV±ß1 œPLã'"SʍAèNƒ¾gñ‹ÒÒ6"WL*ì¯óç«
×V'àí™ß÷Z¡Ý‰]ÞÛeHQ'ã¶ë~[vÔvƒ—ÚÁ<‰¦Ï¨¢¨5FÏU6êJD.ÖÌûÒÉ+ ÀNQQQçLwȲ ý°RàKÝ)¦ZŸô÷Äu1S6ˆ²6±5$Ø)1Š¯a
ôÉÜ!_ ºÕg¦`Ñφ½>^*pàå_û!óñïD4¾zÀFÏ'Î#€£¼[Ø¿«œȸÿ×LÍÀ	["Š<ek¾`Kӊ4@fB|ÚÖO–Wtû¾½)
؁ͯý7l«°C=Γí©Ï},^ëdXôY(¨"³"ÅÍEž6¦½¡ÊP5R$Á½u3"$ÃU$BÛB¤ü_>j:JNU"&"mÞ3m¤
¹÷îMäÄ)<#Ò+ômµ ` ·6/¤ ÕäƒÓjB'#I8úx=֛Ž¤¡&bӔ]üðýÅj÷ù'¾L'øœû°Ñ«Xö—úA. }ŒÇ—·Yùùm‰ábç"óÎÞU'Ðü`æ¥ZÿLÆ<ú@H@½ÙÌ·Õí3¯e¹~ý:¼15Ñ
=PdïdÓÿ¥T™w¿ú¯C6
š;‡"Ë쑩š[lÕ†ž*´ôЫ÷Ic*6h
ZËÐF—è¨<ã~ex©a?@¿í‡î½Ð?¬ƒ÷Ý¥ûž]Iè°(íFWz³§ggoÆZk€†Õò¶óŠàëÃN—=¡mEèhÍldûDÆî[™GL´9ó=Û\
§£·/ÃÙ$"Èôšz;àÔË ¾½øþ¡ªÜÖ×;>VN[óÿ9†êÑ‡²ïÑ;Å·@õ:×éîäHÅÇ–#¡3֕¾Ñ6AXîïÏ®.M4‹}Ü'&g
I5`Ä&P·l
w¯¡Qõt!Õ?¾£—¥;^vˆ§Ð¡eû8Áns7cãÐ>iô~@ÔøÛ·'êl²½·"7¿{ä°:½š«ßvxËß¡K¸
ýPà¿5JŠÞòŽQ'Xžº¯ÎnÆn³)è!ÊA»<"éS¥ž¢­©©"Þ܇v]ûÑ#½'Z3›¾'!¹B&"TNÓÞ|ûQþ—ý—ý'
PòçE6æÅúÓ®
-摄zpºãr.8"¢GóÒ¥VÛe%Â<µÚwn‡å'§** ÃÝ']Oâp†ºlÖ~/'•(˜	BwÑ5›z›º$¬ŠQßþ¤r£'ï°
ÁlŠÒóö#›¡'%ÍÀ°ÊÿØy¸ó"!è$:ºÐmY5ès¸,ŽœÐŽ"")ü¸ÐH|F£aÍsƒÄšÉÍË#:¸ñûøԐ¸¥j?›pBA	Øüó8þ?ÉP7,ÎÊÒ¬ZôHÄ~o{+EÄR$=P°­¹ÍÖ*{ñW'èéqx1ã5zjI$ÝÚ_mO,Â/×.úÖ½Ô{M× ÐAóD,J¢/c£™PPª2#¢¹•™¢êhs¢ü˜c‹!ºµg:Vl†æüɐÁwŸbGàèï°}LX:Ua fðÐ0QŒ¾oBÁÄì¾Î&ü1šp%æCw/"ÁÓ Ê[M´ÁÜo!:²í;{ê¿vmýÓ§ÃQ¨á(;q·èGj¿®&¼Ù9ٕŸ_•PLqát¯œƒ±Aь³wÓÊtÛëMôy}¾êí¥€tô 2ÑG^u+«,Lm­:
È<€øŸU2ȡՄ­sº%"ÔÛ²ÃÃû™'|žÞ}ròPH`Õäh…ñkG|"PøõA²æÄ̗NBôú!¦lƒ£ûÄï'z³š"
Î}&o–$> ñé"-ºûÑã(ÛcURêiu'FèuM¼‰xy<į*¨¬#؆š‹ý›!]iÅãÉýj%6áKœ¡=S65ÙՖMÙÕÈ>åÑÖª¿2°Œ} ZDZcPdÅ¡j̶?
tܲ.døV'ÑhZ-{´ZŽ†–Ví·Š¡·è¤sƵ¨ëf=#ۉ'#¨ÊcØhÞiCÑKrãÕS»ù&¡ë"E6Š"­;±"¸ÕÛô† Ü£Ùuž#¬€áÛøìŸG…2'ƒøÒB'gï•UP'ð@ÖßÎX€Ä|sÕ Ãíî¶RnU&¢ÚATBhMÑÜ:ý³UÕ A»€
×h/§/ L@÷¨råææZâ4wtw‡'Ð`Jb¼®æ
íKº¼3<=Û£!FéuHð¡3ö®Ú‰Ü_ºB¾ˆÏÈTq0¾2L6
jø#Œ"Hª/¾Û?²ø^¸PÖó+;œ-r8ᇙYhC‰ïJÐsŠ)uDŸ9!3"Xµ}gŸŠ‹µ{?÷"îObeU•
']4‡vM*Ãi…måéäÚ.n€^%|šáᏗOyù¶/ö¤~œH-o?tGòPò%ú–rÉk™%.[Ú\1QNn2r'7,­=]o1ç\ü™oZkî'Q)G#òÆM
ƒl†-å;Ë$ÙÙcŽ>n?Ðs¸þ›/m›-ÃáÕ1K¹ZoòõkJßÖ³òÇÿå÷ïs+ûÒìŠT2ѽŸ	nÂSø]‰‹tS8ß9'×NA©áœ²iíßôf‡9%‰6†÷ïwì§GPÚͼdÂŽmZ¾½½ý£êj¡>éÉEo'.±?F™ãàôr"ÁÍÁzbïÁ;UT$Ô3j›úqÔc''–ƒ³³^™ÞãK¢,´Â¼q`itŸÛ>´·9"œ÷þ½iwO"j¨²¾‹RÈXùô~Ôlâs["Wr%´•¿t#jñÒØ3*°¦Z'Ìß}ëS®e2ÑSgúzh‹§ôõ÷'ü]TŸüá£é¤‡ú~¹‰¶4ª}ýÂ%Tû£%74"Š˜š´îZ*Ód£Bæõ¶Ìmoz¤u3ä<¢JŠ¨ÉéŒv1ÒLׯŒô½)>½ãºšOã›[Ë	n\|ðÎzÛxå_}ýztüî~
'þ_–¡™5
` ¤Hbd¥§åх.lð±'H'H`é#OúÀµ3XùÂS†…§nڙ&uwc'©§{p஼ÔٓƒÔì{'Щ¬Eëë#Or@==—ÖM¶íøAñN
‹'{?"üP]õ{šfžÝ]qél²Ãŋ/æƒÎ3®xÐ7¿B7i¢Îž$­¼!ñÍÇvˆ$iA'ÂÉÁáZÇby'RìÔlÓ,NWZj*þŠÌH0³§¸¾ÞÅüq´†]:ª(YgÏA…'³ƒ=|-'ó¬Æøðé›Î?‡®:¶öÑ•¢ÞÏ&aÑÿìYðÃ÷÷'É\4÷$¼îè )}§¬»Ó2k¤'õh­úþg팙©Ž›lðÂZÿú^vÐPš•P¿ã¤`u³bǸ^£«­dfÆ¡ª‹¼Œáû¯'gΜ'–—ÿê)ÜH7&ÀQïĉ8"ñe°ªB©:R‰,'gHgÚãøÎKqdæëÏ5ˏf"(2s´³ks#"íx|É®Âôzl,s‰~Ié—Ÿ¥íŽ¸»•…–êà¡C@i‰Yå"býOÖ×®ÇÅ¥z)rîcs'º'CBB8ÙÙ]° l6[Yg•¡h	üç.hå::;{Ö	'=%žbgš¬¦®nÇNݳ³ŸJΤ€+Ìꂷ·Éæm¼ý/^Пë=Æ°_÷äs[Ã]»v%±]Ù´ZÛ÷þ}ᏩÑ½
rÞÃ/\ïOdÈåá˵æ[Ge)XgoöLõ­®Vãˆæ
ךÛñ|Ò
6!‡Ï¹€"År—RªKëüþóçM__NÂ…Ì@ÆÎ)"_/sòò2û™"ZËFJBz³¼´4LҀ3Ù;…T5°y666×D¿ÒÊÊl¾V@1¾Ös.MéùdTÐ盛Ž˜Í˜Ë»9· KÇ7ÓÑÚÏޏa<@©ÒÁÑkñ|îfP­]Z>°æA99­êg±Äe†—/—ÖÖÕ-£Ñëâ–Öž­ÿºa¡ààc`€|$Ö¯"<Ś÷"ðE¡}_>T:á|FµZ;§Põ?"É=ÈÊâË£9[ù«77HÐ'¾W®˜¢´¸é†kÑf[|MÔroŽÝ_U❵µKèt´²ºjwܒέ&5¨¿º>ò3yLÔ)îŒþøEÂ`!þhBIé'ÖµNìî¬IrœJ叶^¢ºNÕÉÏÏ,ŽOñ-Û9¿,ØÙéYOÓ /å2ŒP;ß\pfÉýjf9´ÅPL+=z4-=ýÔ¡Ûu';¾4åå©^®_f£]¶$?ûjp°øÎ^]ÖÖʈU´"˜òÅ褤$Ò4ø'çŠ~z
Ö2U"‹‹þ¦M›~£ÛäàáÅ*Mé|ý°:ˆéØðçûéqniOPRq"eAàpá'ÆöíÛm"±%"+†Å\T0\˜0,õ0ÍAêë
A°Ÿe$¥èù0ˆ×bq«
}°P·*†9Ϧõ™÷aRYйŽ‰ÅiðÈ\÷øóóF_PSc¯Ñ2×´Ïô̙^öW]")ÈÃËÈÂÙòq§ñA¦Z¯…;ÎCÕY.²÷Qd©ÒÞtÇ@<¥²¶¶‹À£0˪=ÞHaqu~ÞÙÃËË) Àâ£ßëZy7o>&¯Oé*4w²´:ý¬"'œÎ;X›°gxxó†󕅏ç3YÍÊáÔñàØ¢¬¬&â©ØíÇJ°W PÙp»ºÌå'S²ÜÆò¼^uÒýå0Ç>éÊ++ó÷•lò^¦1i<$E™×ôÙp KèÄ5Ös–<A§gjnn´"ñUc#?¯Ë–ÓAÚH¡=ð©š÷<®9üÔÿlž¡f¤J°Þ&ñ"‡´çãbyvþi´£k´Ã^'4ýùTjLÀêØæî/"X£])˜‹O‰gè‰òÆ}_Ž¡&/¢	Q»*'/ŠªžššB'¼'¤zœÄÉY}±.Cìèñã!ć3¢
;¿8Ìpj›œÉ±$dkÅÜ9KÓñ {óòv˝=¢_cF¬‹!?¬bX|Kã9¥F
ÇcØuøK¤wíéËóžï1æa>ƒÉ
2¿¬½eJÕÏNÁªos‡þ,<†×ü¾Ã"Ž×ãs‡÷˜œLðÔr"Sò¼X˜­»a‹ºôýe ~xäH(b֘½®óòX™7PR"ÂB[XY™4o¼£kêG§­vzš0©-Ç2FÏIéïŗ¾~ÿþ~½—X{áQAºç§Pª!ˆìnÖ-éÈÙ,}}¹(pŒ0ôÀ@Žÿ'þv®>¦­*Š?ȍ‹Šå£
ÌR>eë""b]]6a£Œ²…"­0Ö¦ˆµë tÙ2Ç(+H1
ˊÅ™m­€¥0¾¶c"
Ž2
B¡óÔ¿ÝÆM^^òúîé;÷œsÏïœ{ï¹o"µÎKFLÌÌ4¸¸ºœ0‰dŠŃÙ0h§yåLsu®@Êc±'éttñ'oiÁ™Ìːď߀+L'É/¦¸â·QÍ*×;6HT¿B'…Ö@Á'˜AƒÛ&8¾
CÒCKàVó€ÚøôtÛÊÊJ¿*-´Ö	a,x‹WâAK†êâóõ"·j¯G'>BÙ̕õ¡-á9qäp/ȤjÀya'ûç•~D¾|{ûc`!¸np­?õ\Ù;°­
Jɺ©ª'Ð@ gÁì8Ø3ŒmØÞ;n2Ý]à	8ìvd§˜ü*+R–¹=p+…˜§¶Yâ$5¾nTfѪð)Ηâ'ÙZp¨ÒûE]¸Üå7l{û]Ê ·Ž°©oÎg?²6êFE2Rákp?Þ×¼Å2?XZj}ŒX%c—?@ð«œËaC^É2Ch&F6b"g'_¾aTbÎA½›¡Ø'	"<®ÃÆGEµëÐÚ`}§» ¥7Õs.®Îx'kþ|7œ|*(ï€ …^Nî¢=»¿]~±î>½
§#ºg¼ïÂ%œ׿EÆÂ}¦ðþáEDŽ‡C7ÿ'p¡'R¼î<:o3c¢ç	"?ænbŤ¾
å%˨q™"µ)¡%sn'«!$;!Èx;©qí1Ù\oýQ"Ï ÓRM×%Žæ¦õìZCx AÈæÌY¥"¼è<°'/ijV~îyKíBöDRûr† ZÄÖ©h ÒJÆgoýô¸×Hö÷ÚEÁ:…'k±Â{õþ#â¥ºiø —8ꓧö<ÓVQš~rcPËéÞ~CŠÒä¤X…!š;Ν ôSêR h­eÐvž,›±±Ýºi%Óv«I³¯õÀ´í*ÔÏÏã0È܏QdTžu8¤t–5̝Œæ±¡‡R"¯p¾Ÿ³xåºøÔ¡´Ê¨{ýÂR+ÿ‹Ï§Ø/{¿	•©Ôá64?±"Áè0'1ôöYŽQmný²zñâ€Rž/z툭ª±jYÈî'H<Ü\Àú†ø HCêÍ«d@PiMêæI–ºñÓô^¥\³7Ó/&¶Ñ‹³/Lhì+\O"Ù~€"E0ÌYډ`ã¾f5ƒöàL¬$'i[µÛ×çŸò×g›§C¥˜Þ¯â7
†è qÉ×,Û,1í»]k¯wý`ìžN<ùÙ9KüeYSHÔìû½hc5@TMûVT?¦+ÕìmvL©÷†"¯]ñRÜ$ÑÿªÈ>©"Ó·òêC
vàؽºežÝ÷ƒ1³;E8òfng"6w:eòÀnD±¦6›Ò­BRJXúÝo¤[ÏÛÑ9xõá](9AN8v‡"Yú$¥<ò

==> 2106.03898v3_Shmakov/supmaterial.tex <==
\pagebreak

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}

\section{Appendix A: Symmetric Tensor Attention Proofs}
\begin{theorem}
Given a permutation group $G \subseteq S_k$ for any integer $k$, a rank-$k$ parameter tensor $\Theta \in \mathbb{R}^{D \times D \times \dots \times D}$, and a set of input vectors $X \in \mathbb{R}^{N \times D}$ the following set of operations
\begin{align}
     \mathcal{S}^{i_1 i_2 \dots i_{k}} &= \sum_{\sigma \in G} \Theta^{i_{\sigma\left(1\right)} i_{\sigma\left(2\right)} \dots i_{\sigma\left(k\right)}} \label{tap_p1} \\
     \mathcal{O}^{j_1 j_2 \dots j_{k}} &= X^{j_1}_{i_1} X^{j_2}_{i_2} \dots X^{j_{k}}_{i_{k}}  \mathcal{S}^{i_1 i_2 \dots i_{k}} \label{tap_p2} \\
     \mathcal{P}^{j_1 j_2 \dots j_{k}} &= \frac{\exp{(\mathcal{O}^{j_1 j_2 \dots j_{k}})}}{\sum_{j_1, j_2, \dots, j_{k}} \exp{(\mathcal{O}^{j_1 j_2 \dots j_{k}})}} \label{tap_p3}
\end{align}

will produce a an output tensor, $\mathcal{P}$, that is $G$-symmetric. That is, 
$$\forall \sigma \in G,\ \mathcal{P}^{j_1 j_2 \dots j_k} = \mathcal{P}^{j_{\sigma(1)} j_{\sigma(2)} \dots j_{\sigma(k)}} $$
\end{theorem}

\begin{proof}
In order to prove that the output, $\mathcal{P}$, is $G$-symmetric, it is sufficient to prove that every step produces a $G$-symmetric tensor. We will now prove that the result from all three steps will be $G$-symmetric.

\begin{itemize}
    \item We will first prove that the output to Equation \ref{tap_p1}, which is known as the (unnormalized) \textit{symmetric part} of tensor $\Theta$, will be $G$-symmetric. That is,
    $$\forall \tau \in G,\ \mathcal{S}^{j_1 j_2 \dots j_k} = \mathcal{S}^{j_{\tau(1)} j_{\tau(2)} \dots j_{\tau(k)}} $$
    Since $G$ is a group, for every element $\nu \in G$, there exists a unique $\sigma \in G$ such that $\nu = \sigma \tau$. This is a consequence of the unique inverse property of groups, forcing that element to be $\sigma = \nu \tau ^ {-1}$. Therefore,
    \begin{align*}
        \mathcal{S}^{j_{\tau(1)} j_{\tau(2)} \dots j_{\tau(k)}} &= \sum_{\sigma \in G} \Theta^{i_{\sigma\left(\tau(1)\right)} i_{\sigma\left(\tau(2)\right)} \dots i_{\sigma\left(\tau(k)\right)}} \\
        &= \sum_{\nu \in G} \Theta^{i_{\left ( \nu \tau^{-1} \tau \right )\left(1\right)} i_{\left ( \nu \tau^{-1} \tau \right )\left(2\right)} \dots i_{\left ( \nu \tau^{-1} \tau \right )\left(k\right)}} \\
        &= \sum_{\nu \in G} \Theta^{i_{\nu\left(1\right)} i_{\nu\left(2\right)} \dots i_{\nu\left(k\right)}} \\
        &= \mathcal{S}^{j_{1} j_{2} \dots j_{k}}
    \end{align*}
    
    \item For Equation \ref{tap_p2}, we use the same $X$ tensor $k$ times in the expression. Since these tensors are all identical, they are trivially symmetric since and we can freely swap the order of the $X$ tensors as long as we apply an inverse permutation to another set of indices. Furthermore, since $\mathcal{S}$ is $G$-symmetric from the previous step, it can also freely permute its indices according to $G$. Therefore,
    \begin{align*}
        \forall \sigma \in G, \mathcal{O}^{j_{\sigma(1)} j_{\sigma(2)} \dots j_{\sigma(k)}} &= X^{j_{\sigma(1)}}_{i_1} X^{j_{\sigma(2)}}_{i_2} \dots X^{j_{\sigma(k)}}_{i_{k}}  \mathcal{S}^{i_1 i_2 \dots i_{k}} \\
        &= X^{j_1}_{i_{\sigma^{-1}(1)}} X^{j_2}_{i_{\sigma^{-1}(2)}} \dots X^{j_k}_{i_{\sigma^{-1}(k)}}  \mathcal{S}^{i_{1} i_{2} \dots i_{k}} \\
        &= X^{j_1}_{i_{1}} X^{j_2}_{i_{2}} \dots X^{j_k}_{i_{k}}  \mathcal{S}^{i_{\sigma(1)} i_{\sigma(2)} \dots i_{\sigma(k)}} \\
        &= X^{j_1}_{i_{1}} X^{j_2}_{i_{2}} \dots X^{j_k}_{i_{k}}  \mathcal{S}^{i_{1} i_{2} \dots i_{k}} \\
        &= \mathcal{O}^{j_{1} j_{2} \dots j_{k}}
    \end{align*}
    
    \item For Equation \ref{tap_p3}, the operations are performed element-wise to every element in $\mathcal{O}$ and the normalisation term is simply the sum of all elements in $\exp(\mathcal{O})$. Since summation is commutative, 
    $$ \forall \sigma \in G, \ \sum_{j_1, j_2, \dots, j_{k}} \exp{(\mathcal{O}^{j_1 j_2 \dots j_{k}})} = \sum_{j_{\sigma(1)}, j_{\sigma(2)}, \dots, j_{\sigma(k)}} \exp{(\mathcal{O}^{j_{\sigma(1)} j_{\sigma(2)} \dots j_{\sigma(k)}})}$$
    
    Combining the fact that both the normalisation term and $\mathcal{O}$ are both $G$-symmetric, we find that the output is also $G$-symmetric.
    \begin{align*}
    \forall \sigma \in G,\ \mathcal{P}^{j_{\sigma(1)} j_{\sigma(2)} \dots j_{\sigma(k)}} &= \frac{\exp{(\mathcal{O}^{j_{\sigma(1)} j_{\sigma(2)} \dots j_{\sigma(k)}})}}{\sum_{i_{\sigma(1)}, i_{\sigma(2)}, \dots, i_{\sigma(k)}} \exp{(\mathcal{O}^{i_{\sigma(1)} i_{\sigma(2)} \dots i_{\sigma(k)}})}} \\
    &= \frac{\exp{(\mathcal{O}^{j_1 j_2 \dots j_{k}})}}{\sum_{i_1, i_2, \dots, i_{k}} \exp{(\mathcal{O}^{i_1 i_2 \dots i_{k}})}} \\
    &= \mathcal{P}^{j_1 j_2 \dots j_k}
    \end{align*}
\end{itemize}

\end{proof}

\subsection{Run-time Complexity}
For the following sections, we will treat the network's hidden representation dimension $D$ as a constant. This is because this value is a hyperparameter which may be adjusted freely, although we also provide the run-time expressions with $D$ present.

\begin{itemize}
    \item Equation \ref{tap_p1}. This expression is simply an element-wise sum over all possible elements of group $G$ and tensor $\Theta$. The run-time of this step is therefore exponential with respect to the number of partons in each partition.
    \begin{align*}
        O\left(|G|D^k\right) &= O\left(k! D^k\right) \\
        &= O\left(k^k D^k\right) \\
        &= O\left((Dk)^k\right) \\
        &= O\left(k^k\right)
    \end{align*}
    
    \item Equation \ref{tap_p2}. This expression evaluates a generalized tensor-product between $k$ rank-$2$ tensors and one rank-$k$ tensor. The output will be rank-$k$ tensor with sizes $N \times N \times \dots \times N$. For each of these outputs, the operation must perform a rank-$k$ tensor multiplication with sizes $D \times D \times \dots \times D$. The run-time of this step is therefore exponential with respect to the number of partons in each partition. We note that this is only the naive run-time and many tensor-multiplication libraries will not use divide-and-conquer algorithms to reduce the $O\left(D^k\right)$ multiplication operation.
    \begin{align*}
        O\left(N^k D^k\right) &= O\left((ND)^k\right) \\
        &= O\left(N^k\right)
    \end{align*}
    
    \item Equation \ref{tap_p3}. The normalization factor can be pre-computed once for every element of $\mathcal{O}$. This expression then reduces to simply an element-wise exponentiation and division over all $O\left(N^k\right)$ elements in $\mathcal{O}$
\end{itemize}

The total run-time complexity of the symmetric tensor attention layer assuming that $D$ is constant is therefore simply
$$ O(k^k + N^k) $$

\section{Appendix B: SPANet Modifications}

\subsection{Soft Loss Function}
When constructing the symmetric loss function, we use the minimum loss over all equivalent particle orderings as our optimization objective. However, this might cause instability on events where the network is unsure, causing the loss function to flip every epoch for that event. In order to prevent this and maintain a continually differentiable loss function, we use a modified loss based on the $\softmin$ function.
\begin{align*}
    \mathcal{L}_{softmin} &= \softmin_{\sigma \in G_E} \sum_{i = 1}^m CE(\mathcal{P}_i, \mathcal{T}_{\sigma(i)}) \\ \text{ where } \\
    \softmin{\{x_1, x_2, \dots, x_k \}} &= \sum_{j = 1}^k \frac{e^{-x_j}}{\sum_{i = 1}^k e^{-x_i}} x_j
\end{align*}

\subsection{Balanced Loss Scaling}
We experiment with balancing the loss based on the prevalence of each combination of particles in the target set. This is primarily to prevent the network from ignoring rare events such as the complete \tttt{} event when performing partial event training. If there is a large imbalance between classes, such as when events with fewer particle are more prevalent, this could cause the network to bias its results towards those more common events and worsen performance on full events. 

We compute the class balance term $CB(\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m)$ where the $\mathcal{M}_p$ terms represent binary values indicating if a particle $p$ is present or not in the event and $m$ is the total number of particles. If $\mathcal{M}_p = 1$, then $p$ is fully reconstructable in the given event, and if $\mathcal{M}_p = 0$, then at least one parton associated with particle $p$ is not detectable.

Assume we have a dataset of size $N$ of such events, each with their own masking vector for each possible particle $\mathcal{M}_p^j$ for $1 \leq j \leq N$ and $1 \leq p \leq m$. We will keep the particle indices in the subscript and the dataset indices in the superscript. Assume we also have an \textit{event-level} permutation group $G_E \subseteq S_m$ (Section \ref{sec:arch}). We define $CB$ based on \textit{effective class count} \cite{class_balance}.

First, we will define a counting function. Let $\mathbbm{1}_{P}$ be the selection function for prediction $P$. This is, 
$$ \mathbbm{1}_{P} = \begin{cases} 
      1 & \text{ if } P \text{ is } True \\
      0 & \text{ Otherwise}
   \end{cases}
$$
Next, define label-counting function $C$ which simply counts how many times a particular arrangement of masking values appears in our dataset.
$$C(\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m) = \sum_{j = 1}^N \prod_{p = 1}^m \mathbbm{1}_{\mathcal{M}_p^j = \mathcal{M}_p}$$
Such a counting function does not account for the equivalent particle assignments that are induced by our event-level group $G_E$. To accommodate particle symmetries, we create a symmetric counting function $S$ which counts not only the presence of any particular arrangement of masking values, but also all \textit{equivalent} arrangements.
$$S(\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m) = \sum_{\sigma \in G_E} \sum_{j = 1}^N \prod_{p = 1}^m \mathbbm{1}_{\mathcal{M}_p^j = \mathcal{M}_{\sigma(p)}}$$
Notice that this definition guarantees that any two equivalent masking value sets will have identical symmetric class counts.
$$ \forall \sigma \in G_E,\  S(\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m) = S(\mathcal{M}_{\sigma(1)}, \mathcal{M}_{\sigma(2)}, \dots, \mathcal{M}_{\sigma(m)})$$

We set the scale $\beta$ in effective class definition based on the size of our dataset $N$.
$$ \beta = 1 - 10^{-\log_{10}N}$$

Finally, We define the class balance ($CB$) as the normalized values of the effective class counts ($ECC$) \cite{class_balance}
\begin{align*}
    ECC (\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m) &= \frac{1 - \beta^{S(\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m)}}{1 - \beta} \\
    CB (\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m) &= \frac{ECC (\mathcal{M}_1, \mathcal{M}_2, \dots, \mathcal{M}_m)}{\sum_{\mathcal{M}' \in \{0, 1\}^{m}} ECC (\mathcal{M}'_1, \mathcal{M}'_2, \dots, \mathcal{M}'_m)}
\end{align*}    
$$  $$

\section{Appendix C: Hyperparameters}

\begin{table}[H]
\centering
\begin{tabular}{l|lll}
\hline
\hline
\textbf{Parameter} &\multicolumn{3}{c}{\textbf{Benchmark Problems}} \\
                  & \ttbar{} & \ttH{} & \tttt{} \\ \hline
Training Epochs            & 50 & 50 & 50  \\
Learning Rate              &  0.0015 &   0.00302 &   0.0015  \\
Batch Size                 &  2048  & 2048 & 2048 \\
Dropout Percentage         & 0.1 & 0.1 & 0.1 \\
$L_2$ Gradient Clipping    & N/A & 0.1 & N/A \\
$L_2$ Weight Normalization & 0.0002 & 0.0000683 &  0.0002 \\ \hline
Hidden Dimensionality      & 128 & 128 & 128 \\
Central Encoder Count      & 6 & 5 &  2 \\
Branch Encoder Count       & 3 & 5 &  7 \\ \hline
Partial Event Training     & Yes & Yes & Yes \\
Loss Scaling               & Yes & Yes &  Yes \\
Loss Type                  & $\mathcal{L}_{\min}$ & $\mathcal{L}_{\softmin}$ & $\mathcal{L}_{\softmin}$ \\
Cosine Annealing Cycles    & 5  & 5 & 5 \\
\hline
\hline
\end{tabular}
\caption{A complete table of all hyper-parameters used during \spanet{} training on all benchmark problems.}
\end{table}

\section{Appendix D: $\chi^2$ Method Details}

In Section~\ref{sec:chi2}, we introduce the $\chi^2$ method for reconstructing \ttbar{} events. This is a standard benchmark against which we can compare the results from \spanet{}, and has been used in multiple published results, such as ~\cite{Aaboud:2017mae, Aad:2020nsf}. However, no such benchmark exists for the \ttH{} and \tttt{} topologies. We thus extend the $\chi^2$ method to these topologies in a simple way in order to have a benchmark to compare against. 

The \ttbar{} formulation we use is given in Equation~\ref{eqn:chi2ttbar}. In \cite{spanet1}, a different formulation of $\chi^2$ was used that more closely matches recent ATLAS results in which $\sigma_t$ is not used explicitly. While this formulation reduces mass sculpting of incomplete and background events, it does not perform well on events partial events with only a single reconstructable top quark. Further, it is unclear how to optimally extend this formulation to the \tttt{} case. Thus, in this work we prefer the formulation that explicitly includes $m_t$.

The $\chi^2$ is evaluated on \ttH{} events as:

\begin{align}
              \chi^2_{\ttH} &= \frac{(m_{b_1q_1q_1} - m_{t})^2}{\sigma^2_{{t}}} + \frac{(m_{b_2q_2q_2} - m_{t})^2}{\sigma^2_{{t}}}\nonumber \\ &+  \frac{(m_{q_1q_1} - m_W)^2}{\sigma^2_{W}} +\frac{(m_{q_2q_2} - m_W)^2}{\sigma^2_{W}} + \frac{(m_{b_0b_0} - m_H)^2}{\sigma^2_{H}} ,
     \label{eqn:chi2ttH}
\end{align}

where we have simply added an additional term to Equation~\ref{eqn:chi2ttbar} for the Higgs boson, analogously to the terms used for the $W$-bosons. We label the jets hypothesized to be the decay products of the Higgs boson as $b_0$ here and find $\sigma_H = 22.3$~GeV in our dataset.

The $\chi^2$ for \tttt{} is given by the expression

\begin{align}
          \chi^2_{\fourtop} &= \frac{(m_{b_1q_1q_1} - m_{t})^2}{\sigma^2_{{t}}} + \frac{(m_{b_2q_2q_2} - m_{t})^2}{\sigma^2_{{t}}} + \frac{(m_{b_3q_3q_3} - m_{t})^2}{\sigma^2_{{t}}} + \frac{(m_{b_4q_4q_4} - {t})^2}{\sigma^2_{t}} \nonumber \\
          &+ \frac{(m_{q_1q_1} - m_W)^2}{\sigma^2_{W}} + \frac{(m_{q_2q_2} - m_W)^2}{\sigma^2_{W}} + \frac{(m_{q_3q_3} - m_W)^2}{\sigma^2_{W}} + \frac{(m_{q_4q_4} - m_W)^2}{\sigma^2_{W}} ,
     \label{eqn:chi24top}
\end{align}

where we have simply added additional, identical terms for the third and fourth top quarks and $W$-bosons. We find that the complexity of the 12 parton final state makes this effectively intractable and thus do not present reconstruction performance with this formulation, presenting it only as a demonstration that the CPU overhead required in this topology means permutation methods do not scale to these events.

\section{Appendix E: Additional Result Tables}

\begin{table}[h]
    \centering
    \input{tables/ttbar_spanet_pythia}    
    \vspace{0.1cm}
    \caption{\spanet{} results on \ttbar{} using Pythia showering.}
    \label{tab:ttbar_pythia_spanet_full}
\end{table}

\begin{table}[h]
    \centering
    \input{tables/ttbar_py8_chi2_metrics}    
    \vspace{0.1cm}
    \caption{$\chi^2$ method results on \ttbar{} using Pythia showering.}
    \label{tab:ttbar_pythia_chi2_full}
\end{table}

\begin{table}[h]
    \centering
\input{tables/ttbar_herwig}    
    \vspace{0.1cm}
    \caption{\spanet{} results on \ttbar{} using Herwig showering.}
    \label{tab:ttbar_herwig_spanet_full}
\end{table}

\begin{table}[h]
    \centering
\input{tables/ttbar_herwig_chi2_metrics}    
    \vspace{0.1cm}
    \caption{$\chi^2$ method results on \ttbar{} using Herwig showering.}
    \label{tab:ttbar_herwig_chi2_full}
\end{table}

\begin{table}[h]
    \centering
    \input{tables/ttH}    
    \vspace{0.1cm}
    \caption{\spanet{} results on \ttH{} with at least $2$ $b$-tagged jets (all generated events).}
    \label{tab:tth_spanet_2btag}
\end{table}

\begin{table}[h]
    \centering
    \input{tables/ttH_min_4}    
    \vspace{0.1cm}
    \caption{\spanet{} results on \ttH{} with at least $4$ $b$-tagged jets (filtered events).}
    \label{tab:tth_chi2_4btag}
\end{table}

\begin{table}[h]
    \centering
    \input{tables/tttt}    
    \vspace{0.1cm}
    \caption{\spanet{} results on \tttt{} with at least $2$ $b$-tagged jets (all generated events).}
    \label{tab:tttt_spanet_2btag}
\end{table}

\begin{table}[h]
    \centering
    \input{tables/tttt_min_4}    
    \vspace{0.1cm}
    \caption{\spanet{} results on \tttt{} with at least $4$ $b$-tagged jets (filtered events).}
    \label{tab:tttt_chi2_4btag}
\end{table}


==> 2106.03898v3_Shmakov/tables/ttH.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction & Event Efficiency & Higgs Efficiency & Top Quark 
Efficiency\\
\hline
All Events&== 8 & 0.281 & 0.329 & 0.430 & 0.498\\
&== 9 & 0.316 & 0.304 & 0.430 & 0.476\\
&$\geq 10$ & 0.355 & 0.264 & 0.420 & 0.441\\
&\textbf{Inclusive} & \textbf{0.954} & \textbf{0.297} & \textbf{0.426} & \textbf{0.468}\\
\hline
\hline
Higgs Events&== 8 & 0.197 & 0.317 & 0.430 & 0.531\\
&== 9 & 0.227 & 0.295 & 0.430 & 0.504\\
&$\geq 10$ & 0.261 & 0.257 & 0.420 & 0.462\\
&\textbf{Inclusive} & \textbf{0.686} & \textbf{0.287} & \textbf{0.426} & \textbf{0.493}\\
\hline
\hline
1 Top Events&== 8 & 0.167 & 0.314 & 0.413 & 0.466\\
&== 9 & 0.177 & 0.297 & 0.409 & 0.448\\
&$\geq 10$ & 0.184 & 0.273 & 0.397 & 0.421\\
&\textbf{Inclusive} & \textbf{0.529} & \textbf{0.294} & \textbf{0.406} & \textbf{0.444}\\
\hline
\hline
2 Top Events&== 8 & 0.066 & 0.352 & 0.590 & 0.539\\
&== 9 & 0.092 & 0.295 & 0.540 & 0.504\\
&$\geq 10$ & 0.130 & 0.225 & 0.490 & 0.456\\
&\textbf{Inclusive} & \textbf{0.289} & \textbf{0.277} & \textbf{0.526} & \textbf{0.490}\\
\hline
\hline
Full Events&== 8 & 0.036 & 0.440 & 0.590 & 0.599\\
&== 9 & 0.057 & 0.344 & 0.540 & 0.542\\
&$\geq 10$ & 0.087 & 0.248 & 0.490 & 0.480\\
&\textbf{Inclusive} & \textbf{0.180} & \textbf{0.317} & \textbf{0.526} & \textbf{0.523}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/ttH_min_4.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction & Event Efficiency & Higgs Efficiency & Top Quark Efficiency\\
\hline
All Events&== 8 & 0.260 & 0.370 & 0.497 & 0.540\\
&== 9 & 0.313 & 0.343 & 0.492 & 0.514\\
&$\geq 10$ & 0.397 & 0.294 & 0.472 & 0.473\\
&\textbf{Inclusive} & \textbf{0.972} & \textbf{0.330} & \textbf{0.485} & \textbf{0.502}\\
\hline
\hline
Higgs Events&== 8 & 0.209 & 0.380 & 0.497 & 0.580\\
&== 9 & 0.252 & 0.355 & 0.492 & 0.550\\
&$\geq 10$ & 0.320 & 0.302 & 0.472 & 0.501\\
&\textbf{Inclusive} & \textbf{0.782} & \textbf{0.340} & \textbf{0.485} & \textbf{0.535}\\
\hline
\hline
1 Top Events&== 8 & 0.153 & 0.335 & 0.479 & 0.494\\
&== 9 & 0.171 & 0.324 & 0.474 & 0.475\\
&$\geq 10$ & 0.199 & 0.296 & 0.448 & 0.446\\
&\textbf{Inclusive} & \textbf{0.524} & \textbf{0.316} & \textbf{0.466} & \textbf{0.469}\\
\hline
\hline
2 Top Events&== 8 & 0.061 & 0.435 & 0.657 & 0.597\\
&== 9 & 0.096 & 0.360 & 0.601 & 0.550\\
&$\geq 10$ & 0.153 & 0.269 & 0.545 & 0.491\\
&\textbf{Inclusive} & \textbf{0.310} & \textbf{0.330} & \textbf{0.583} & \textbf{0.530}\\
\hline
\hline
Full Events&== 8 & 0.042 & 0.532 & 0.657 & 0.663\\
&== 9 & 0.070 & 0.422 & 0.601 & 0.596\\
&$\geq 10$ & 0.116 & 0.306 & 0.545 & 0.523\\
&\textbf{Inclusive} & \textbf{0.228} & \textbf{0.383} & \textbf{0.583} & \textbf{0.572}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/ttbar_body.tex <==
\begin{tabular}{c | c | c | c c | c c}
\hline
\hline
&&Event&\multicolumn{2}{c|}{\spanet{} Efficiency}& \multicolumn{2}{c}{$\chi^2$ Efficiency}\\
& $N_\mathrm{jets}$ & Fraction & Event & Top Quark & Event & Top Quark\\
\hline
All Events&== 6 & 0.245 & 0.643 & 0.696  & 0.424 & 0.484 \\
&== 7 & 0.282 & 0.601 & 0.667 & 0.389 & 0.460 \\
&$\geq 8$ & 0.320 & 0.528 & 0.613 & 0.309 & 0.384 \\
&\textbf{Inclusive} & \textbf{0.848} & \textbf{0.586} & \textbf{0.653} & \textbf{0.392} & \textbf{0.457} \\
\hline
\hline
Complete Events &== 6 & 0.074 & 0.803 & 0.837 & 0.593 & 0.643\\
&== 7 & 0.105 & 0.667 & 0.754 & 0.413 & 0.530\\
&$\geq 8$ & 0.145 & 0.521 & 0.662 & 0.253 & 0.410\\
&\textbf{Inclusive} & \textbf{0.325} & \textbf{0.633} & \textbf{0.732} & \textbf{0.456} & \textbf{0.552}\\
\hline
\hline
\end{tabular}

==> 2106.03898v3_Shmakov/tables/ttbar_herwig.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction  & Event Efficiency & Top Quark Efficiency\\
\hline
All Events&== 6 & 0.220 & 0.659 & 0.711\\
&== 7 & 0.222 & 0.629 & 0.678\\
&$\geq 8$ & 0.185 & 0.564 & 0.618\\
&\textbf{Inclusive} & \textbf{0.629} & \textbf{0.620} & \textbf{0.672}\\
\hline
\hline
1 Top Events&== 6 & 0.156 & 0.593 & 0.593\\
&== 7 & 0.163 & 0.614 & 0.614\\
&$\geq 8$ & 0.138 & 0.575 & 0.575\\
&\textbf{Inclusive} & \textbf{0.459} & \textbf{0.595} & \textbf{0.595}\\
\hline
\hline
2 Top Events&== 6 & 0.064 & 0.819 & 0.854\\
&== 7 & 0.059 & 0.672 & 0.765\\
&$\geq 8$ & 0.046 & 0.533 & 0.684\\
&\textbf{Inclusive} & \textbf{0.170} & \textbf{0.690} & \textbf{0.777}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/ttbar_herwig_chi2_metrics.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction  & Event Efficiency & Top Quark Efficiency\\
\hline
All Events&== 6 & 0.220 & 0.505 & 0.560\\
&== 7 & 0.222 & 0.442 & 0.488\\
&$\geq 8$ & 0.185 & 0.338 & 0.386\\
&\textbf{Inclusive} & \textbf{0.629} & \textbf{0.434} & \textbf{0.484}\\
\hline
\hline
1 Top Events&== 6 & 0.156 & 0.434 & 0.434\\
&== 7 & 0.163 & 0.442 & 0.442\\
&$\geq 8$ & 0.138 & 0.363 & 0.363\\
&\textbf{Inclusive} & \textbf{0.459} & \textbf{0.415} & \textbf{0.415}\\
\hline
\hline
2 Top Events&== 6 & 0.064 & 0.678 & 0.713\\
&== 7 & 0.059 & 0.442 & 0.553\\
&$\geq 8$ & 0.046 & 0.263 & 0.419\\
&\textbf{Inclusive} & \textbf{0.170} & \textbf{0.483} & \textbf{0.577}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/ttbar_herwig_vs_pythia.tex <==
\begin{tabular}{c | c | c c c c | c c c c}
\hline
\hline
& $N_\mathrm{jets}$ & \multicolumn{4}{c}{Pythia8} &  \multicolumn{4}{c}{Herwig7} \\
& & \multicolumn{2}{c}{$\chi^2$} & \multicolumn{2}{c}{\spanet} & \multicolumn{2}{c}{$\chi^2$} & \multicolumn{2}{c}{\spanet} \\
& & Event & Top & Event & Top & Event & Top & Event & Top \\
\hline
All Events&== 6 & 0.423 & 0.483& 0.643 & 0.696&0.475 & 0.526& 0.659 & 0.711\\
&== 7& 0.384 & 0.455& 0.601 & 0.667& 0.411 & 0.464 & 0.629 & 0.678\\
&$\geq 8$&0.293 & 0.381& 0.528 & 0.613& 0.308 & 0.359& 0.564 & 0.618\\
 &\textbf{Inclusive}  &\textbf{0.385} & \textbf{0.453}& \textbf{0.586} & \textbf{0.653}&\textbf{0.434} & \textbf{0.485}&\textbf{0.620} & \textbf{0.672}\\
 \hline
 \hline
% 1 Top Events&== 6 &&& 0.574 & 0.574&& & 0.593 & 0.593\\
% &== 7 &&& 0.562 & 0.562&&& 0.614 & 0.614\\
% &$\geq 8$ &&& 0.534 & 0.534&& & 0.575 & 0.575\\
% &\textbf{Inclusive}  &&& \textbf{0.556} & \textbf{0.556}&&& \textbf{0.595} & \textbf{0.595}\\
% \hline
% \hline
 Complete Events&== 6 &0.592 & 0.642& 0.803 & 0.837&0.633 & 0.680& 0.819 & 0.854\\
 &== 7  &0.408 & 0.522& 0.667 & 0.754&0.393 & 0.522& 0.672 & 0.765\\
 &$\geq 8$ &0.253 & 0.410& 0.521 & 0.662&0.219 & 0.384& 0.533 & 0.684\\
 &\textbf{Inclusive} &\textbf{0.442} & \textbf{0.542}&\textbf{0.633} & \textbf{0.732}&\textbf{0.503} & \textbf{0.591} & \textbf{0.690} & \textbf{0.777}\\
 \hline
 \hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/ttbar_py8_chi2_metrics.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction  & Event Efficiency & Top Quark Efficiency\\
\hline
All Events&== 6 & 0.245 & 0.424 & 0.484\\
&== 7 & 0.282 & 0.389 & 0.460\\
&$\geq 8$ & 0.320 & 0.309 & 0.384\\
&\textbf{Inclusive} & \textbf{0.848} & \textbf{0.392} & \textbf{0.457}\\
\hline
\hline
1 Top Events&== 6 & 0.171 & 0.355 & 0.355\\
&== 7 & 0.176 & 0.373 & 0.373\\
&$\geq 8$ & 0.175 & 0.348 & 0.348\\
&\textbf{Inclusive} & \textbf{0.524} & \textbf{0.359} & \textbf{0.359}\\
\hline
\hline
2 Top Events&== 6 & 0.074 & 0.593 & 0.643\\
&== 7 & 0.105 & 0.413 & 0.530\\
&$\geq 8$ & 0.145 & 0.253 & 0.410\\
&\textbf{Inclusive} & \textbf{0.325} & \textbf{0.456} & \textbf{0.552}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/ttbar_spanet_pythia.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction  & Event Efficiency & Top Quark Efficiency \\
\hline
All Events&== 6 & 0.245 & 0.643 & 0.696\\
&== 7 & 0.282 & 0.601 & 0.667\\
&$\geq 8$ & 0.320 & 0.528 & 0.613\\
&\textbf{Inclusive} & \textbf{0.848} & \textbf{0.586} & \textbf{0.653}\\
\hline
\hline
1 Top Events&== 6 & 0.171 & 0.574 & 0.574\\
&== 7 & 0.176 & 0.562 & 0.562\\
&$\geq 8$ & 0.175 & 0.534 & 0.534\\
&\textbf{Inclusive} & \textbf{0.524} & \textbf{0.556} & \textbf{0.556}\\
\hline
\hline
2 Top Events&== 6 & 0.073 & 0.803 & 0.837\\
&== 7 & 0.105 & 0.667 & 0.754\\
&$\geq 8$ & 0.144 & 0.521 & 0.662\\
&\textbf{Inclusive} & \textbf{0.325} & \textbf{0.633} & \textbf{0.732}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/tth_body.tex <==
\begin{tabular}{c | c | c | c c c | ccc}
\hline
\hline
&&Event&\multicolumn{3}{c|}{\spanet{} Efficiency}& \multicolumn{3}{c}{$\chi^2$ Efficiency}\\
& $N_\mathrm{jets}$ & Fraction & Event & Higgs  & Top  & Event  & Higgs  & Top \\
\hline
All Events&== 8 & 0.261 & 0.370 & 0.497 & 0.540 & 0.044 & 0.151 & 0.053\\
&== 9 & 0.313 & 0.343 & 0.492 & 0.514 & 0.038 & 0.146 & 0.066\\
&$\geq 10$ & 0.313 & 0.294 & 0.472 & 0.473 & 0.030 & 0.135 & 0.072\\
&\textbf{Inclusive} & \textbf{0.972} & \textbf{0.330} & \textbf{0.485} & \textbf{0.502} & \textbf{0.039} & \textbf{0.146} & \textbf{0.062}\\
\hline
\hline
Complete Events&== 8 & 0.042 & 0.532 & 0.657 & 0.663 & 0.016 & 0.151 & 0.063\\
&== 9 & 0.070 & 0.422 & 0.601 & 0.596 & 0.013 & 0.146 & 0.076\\
&$\geq 10$ & 0.115 & 0.306 & 0.545 & 0.523 & 0.008 & 0.134 & 0.080\\
&\textbf{Inclusive} & \textbf{0.228} & \textbf{0.383} & \textbf{0.583} & \textbf{0.572} & \textbf{0.012} & \textbf{0.144} & \textbf{0.073}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/tttt.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction & Event Efficiency &Top Quark Efficiency\\
\hline
All Events&== 12 & 0.227 & 0.257 & 0.458\\
&== 13 & 0.309 & 0.232 & 0.453\\
&$\geq 14$ & 0.433 & 0.185 & 0.426\\
&\textbf{Inclusive} & \textbf{0.970} & \textbf{0.217} & \textbf{0.441}\\
\hline
\hline
1 Top Events&== 12 & 0.060 & 0.412 & 0.412\\
&== 13 & 0.069 & 0.399 & 0.399\\
&$\geq 14$ & 0.073 & 0.374 & 0.374\\
&\textbf{Inclusive} & \textbf{0.202} & \textbf{0.394} & \textbf{0.394}\\
\hline
\hline
2 Top Events&== 12 & 0.106 & 0.217 & 0.441\\
&== 13 & 0.136 & 0.206 & 0.430\\
&$\geq 14$ & 0.172 & 0.181 & 0.406\\
&\textbf{Inclusive} & \textbf{0.415} & \textbf{0.198} & \textbf{0.423}\\
\hline
\hline
3 Top Events&== 12 & 0.056 & 0.162 & 0.482\\
&== 13 & 0.089 & 0.148 & 0.471\\
&$\geq 14$ & 0.148 & 0.117 & 0.436\\
&\textbf{Inclusive} & \textbf{0.294} & \textbf{0.135} & \textbf{0.455}\\
\hline
\hline
4 Top Events&== 12 & 0.005 & 0.297 & 0.580\\
&== 13 & 0.014 & 0.211 & 0.543\\
&$\geq 14$ & 0.039 & 0.111 & 0.470\\
&\textbf{Inclusive} & \textbf{0.059} & \textbf{0.152} & \textbf{0.497}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/tttt_body.tex <==
\begin{tabular}{c | c | c | c c }
\hline
\hline
&&Event&\multicolumn{2}{c}{\spanet{} Efficiency}\\
& $N_\mathrm{jets}$ & Fraction & Event & Top Quark \\
\hline
All Events&== 12 & 0.219 & 0.276 & 0.484\\
&== 13 & 0.304 & 0.247 & 0.474\\
&$\geq 14$ & 0.450 & 0.198 & 0.450\\
&\textbf{Inclusive} & \textbf{0.974} & \textbf{0.231} & \textbf{0.464}\\
\hline
\hline
Complete Events&== 12 & 0.005 & 0.350 & 0.617\\
&== 13 & 0.016 & 0.249 & 0.567\\
&$\geq 14$ & 0.044 & 0.149 & 0.504\\
&\textbf{Inclusive} & \textbf{0.066} & \textbf{0.191} & \textbf{0.529}\\
\hline
\hline
\end{tabular}


==> 2106.03898v3_Shmakov/tables/tttt_min_4.tex <==
\begin{tabular}{c | c | c | c c c}
\hline
\hline
& $N_\mathrm{jets}$ & Event Fraction & Event Efficiency &Top Quark Efficiency\\
\hline
All Events&== 12 & 0.219 & 0.276 & 0.484\\
&== 13 & 0.304 & 0.247 & 0.474\\
&$\geq 14$ & 0.450 & 0.198 & 0.450\\
&\textbf{Inclusive} & \textbf{0.974} & \textbf{0.231} & \textbf{0.464}\\
\hline
\hline
1 Top Events&== 12 & 0.055 & 0.422 & 0.422\\
&== 13 & 0.062 & 0.414 & 0.414\\
&$\geq 14$ & 0.0684 & 0.388 & 0.388\\
&\textbf{Inclusive} & \textbf{0.185} & \textbf{0.407} & \textbf{0.407}\\
\hline
\hline
2 Top Events&== 12 & 0.101 & 0.235 & 0.461\\
&== 13 & 0.132 & 0.222 & 0.445\\
&$\geq 14$ & 0.175 & 0.194 & 0.420\\
&\textbf{Inclusive} & \textbf{0.410} & \textbf{0.213} & \textbf{0.438}\\
\hline
\hline
3 Top Events&== 12 & 0.057 & 0.200 & 0.513\\
&== 13 & 0.094 & 0.172 & 0.492\\
&$\geq 14$ & 0.162 & 0.136 & 0.460\\
&\textbf{Inclusive} & \textbf{0.313} & \textbf{0.159} & \textbf{0.479}\\
\hline
\hline
4 Top Events&== 12 & 0.006 & 0.350 & 0.617\\
&== 13 & 0.016 & 0.249 & 0.567\\
&$\geq 14$ & 0.044 & 0.149 & 0.504\\
&\textbf{Inclusive} & \textbf{0.066} & \textbf{0.191} & \textbf{0.529}\\
\hline
\hline
\end{tabular}

